A moving fixed-interval filter/smoother for estimation of vehicle position using odometer and map-matched GPS

This paper presents some optimal real-time and post-processing estimators of vehicle position using odometer and map-matched GPS measurements. These estimators were based on a simple statistical error model of the odometer and the GPS which makes the model generalizable to other applications. Firstly, an asymptotically minimum variance unbiased estimator and two optimal moving fixed interval filters which are more flexibles are exposed. Then, the post-processing case leads to the construction of two moving fixed interval smoothers. These estimators are tested and compared with the classical Kalman filter with simulated and real data, and the results show a good accuracy of each of them.

==> endfloat/README <==
This is the readme file for the endfloat package v2.5

This readme was modified on October 2, 1997 but without
updated endfloat itself, instead to fix errors in this file
and in endfloat.ins

It was again modified on March 31, 2006, by Frank K\"uster
<frank@kuesterei.ch> to indicate the license clarification (see below).

It was again modified on December 4, 2011, by Axel Sommerfeldt
<axel.sommerfeldt@f-m.fm> to reflect the changes introduced
with version 2.5 of the endfloat package.

Endfloat is a LaTeX package.  Versions 2.1 and above require
LaTeX2e.

Accompanying files should be:

	README				This file
	endfloat.dtx			Docstrip archive  (essential)
	endfloat.ins			(La)TeX batch file (if you
					    don't know what it is
					    then you DO need it)

============================================================
Overview:
  the package places figures and tables at the end of the document,
  as often requested by journals for non-camera ready submission.

========================================================
Installation:

Run

  latex endfloat.ins

This will produce three files, endfloat.sty, endfloat.drv and efxmpl.cfg .
You can run LaTeX on endfloat.drv for the documentation.
  
You should copy the file endfloat.sty to where you keep
your (La)TeX inputs.  You should read the documentation to find out
more about the example configuration file, efxmpl.cfg.

To produce the documentation, run LaTeX on endfloat.drv (or endfloat.dtx)
a couple of times, and then use the makeindex program (which might be
called makeindx on your system) to generate the index

 makeindex -g -s gind.ist endfloat

Then run LaTeX (at least) two more times to get the index in the table
of contents.

=========================================================
Major changes in version 2.5 since 2.4:
  New commands \DeclareDelayedFloat, \DeclareDelayedFloatFlavor,
  and \SetupDelayedFloat added.
  New package options `tablesonly' and `figuresonly' added.

Major changes in version 2.4 since 2.3:
  Configuration file (with example of getting sidewaystable to work),
  Many new hooks for more user control.  Internal changes.

Major changes in version 2.3 and 2.2 since 2.1:
  Documentation and many internal changes.
  Added options for suppressing "Tables" and "Figures" section heads, for
  switching order of tables and figures.  Use of package options
  generally.

=================================================
Maintainer:  Jeff Goldberg (jeffrey@goldmark.org)
Original author: James Darrell McCauley

Obtaining endfloat:  The necessary files are kept on the Comprehensive
TeX Archive Network (CTAN).  Current CTAN sites are ftp.tex.ac.uk,
ftp.shsu.edu, and ftp.dante.de.  They are also mirrored at other locations.
Once on CTAN, type the command "quote site index endfloat" to
find where endfloat lives.  It is probably in
macros/latex/contrib/supported/endfloat .
Get the whole directory.


=================================================
License and copying:
    endfloat for LaTeX
    Copyright (C) 1992 Darrel McCauley
    Copyright (C) 1994-2011 Jeffrey Goldberg <jeffrey@goldmark.org>

    This program is free software; you can redistribute it and/or modify
    it under the terms of the GNU General Public License as published by
    the Free Software Foundation; either version 2 of the License, or
    (at your option) any later version.

    This program is distributed in the hope that it will be useful,
    but WITHOUT ANY WARRANTY; without even the implied warranty of
    MERCHANTABILITY or FITNESS FOR A PARTICULAR PURPOSE.  See the
    GNU General Public License for more details.

    You should have received a copy of the GNU General Public License
    along with this program; if not, write to the Free Software
    Foundation, Inc., 51 Franklin St, Fifth Floor, Boston, MA  02110-1301 USA

This distribution currently comprises the following files:

README
COPYING
endfloat.dtx
endfloat.ins
endfloat.pdf

The license has been clarified by Jeffrey Goldberg in March 06

=================================================
No Warranty:
There is no warranty.  If it doesn't work right, none of the authors
may be held liable for any direct or indirect damage.  There are
some known bugs (see the documentation), there may very well be
some unknown bugs.

===================================================

